Model-tuning Via Prompts Makes NLP Models Adversarially Robust

In recent years, NLP practitioners have converged on the following practice: (i) import an off-the-shelf pretrained (masked) language model; (ii) append a multilayer perceptron atop the CLS token's hidden representation (with randomly initialized weights); and (iii) fine-tune the entire model on a downstream task (MLP-FT). This procedure has produced massive gains on standard NLP benchmarks, but these models remain brittle, even to mild adversarial perturbations. In this work, we demonstrate surprising gains in adversarial robustness enjoyed by Model-tuning Via Prompts (MVP), an alternative method of adapting to downstream tasks. Rather than appending an MLP head to make output prediction, MVP appends a prompt template to the input, and makes prediction via text infilling/completion. Across 5 NLP datasets, 4 adversarial attacks, and 3 different models, MVP improves performance against adversarial substitutions by an average of 8% over standard methods and even outperforms adversarial training-based state-of-art defenses by 3.5%. By combining MVP with adversarial training, we achieve further improvements in adversarial robustness while maintaining performance on unperturbed examples. Finally, we conduct ablations to investigate the mechanism underlying these gains. Notably, we find that the main causes of vulnerability of MLP-FT can be attributed to the misalignment between pre-training and fine-tuning tasks, and the randomly initialized MLP parameters.

==> sections/1-introduction-old.tex <==
% \section{Outline}
% 1. Prompting is robust compared to fine-tuning a new set of parameters. 

% We test three different hypotheses:
% a. the labels are meaningful (there’s some semantic information about the label “politics”)

% b. (label expansion hypothesis): one can use multiple prompt outputs for labeling one class (“elections”, “politics”, “democracy” → label politics)

% c. the prediction via prompting is better aligned with the pretraining task

% d. new model parameters

% 2. If combined with standard adversarial training the results can be further improved.

% 3. Does prompt expansion or label expansion further improve/degrade clean/robust performance

% 4. Prompting is more effectively robust than fine-tuning, i.e., 
% For any given clean accuracy, robust accuracy via prompt is higher than predicting via CLS 


% 5. Prompting has other advantages such as sample-efficiency.



\section{Introduction}

% \dd{My high-level feedback of the introduction is threefold: (1)  too much capital is spent on basics that people know; (2) it also focuses too much on the actual numbers and improvements (the overall nature of the result is important, the specifics can be discussed later), and (3) the interesting hypotheses and follow-up experiments don't get as much attention.}

% Large language models are trained in an unsupervised manner on large corpora of publicly available data~\cite{devlin-etal-2019-bert, Brown2020Language,zhang2022opt,liu2019roberta}. 
% \dd{Let's refrain from saying that the training is done "in an unsupervised manner". Let's start with something that's more relevant to our work. This line could be applied to thousands of papers.}
\begin{figure}[t]
\centering
\includegraphics[width=1.1\linewidth]{figures/Average_performance.pdf}
  \caption{Comparison of the robustness of various baselines and \ourPrompt averaged across 2 attacks and 3 datasets. This figure demonstrates that \ourPrompt + adv is significantly better than any baseline. \dd{This is better suited for the results section. Introductory figures, generally, explain the "key" insight or the finding rather than a detailed comparison with baselines. } \dd{The font in the figure is too small}}
  \label{fig:mvp}
\end{figure}


% The pre-train, then fine-tune paradigm for language models has resulted in large gains in downstream task performance.
% ; but little focus has been put at evaluating if the fine-tuning strategy could be improved.
% \dd{You could stick the first line to thousands of NLP papers, say something specific to our paper---this is precious real-estate.}\todopm{Updated}
% These models are pre-trained with the task of predicting the next word (given context), or infilling tokens in the input sentence that are masked out. 
% This pretraining procedure leads to an improvement in model performance on downstream tasks, especially in the low data regime.
Pre-trained language models~\cite{devlin-etal-2019-bert,liu2019roberta} have traditionally been
adapted to downstream tasks
% , such as text classification, 
by passing its hidden representations through an untrained multi-layer perceptron, and then fine-tuning the entire model (\linearFTns). Recent works have investigated \emph{prompting} as a means for fine-tuning language models~\citep{Brown2020Language,gao-etal-2021-making}. Prompting converts the classification problem into a problem of sequence completion (or mask infilling) by augmenting the input with a text string that may include candidate examples from the dataset, and cues for the model to complete the sequence (prompt template). The output of the model is matched with respect to a set of candidate answers to make the final prediction (\ourPromptns).
% \dd{The first paragraph is 
% quite generic and common-knowledge at this point, I would suggest to relate this quickly with our work.}
% \ddc{In this study, we focus on classification tasks with word-level adversarial attacks.}{}
% Recent advances in large language models have suggested that a new way of performing text classification via 
% zero-shot \emph{prompting} can also be competitive with previous fine-tuning baselines~\citep{Brown2020Language}. 
% \dd{Have to be careful here: development of larger models  
% does not (in itself) present a new way of performing classification. 
% Just that this mode of inference has become accurate enough to be useful. Further, not being able to load/access large models prevents people to finetune.}
% Prompting converts the traditional classification problem into a problem of sequence completion (or mask infilling), a task that the language models were pre-trained on. This is operationalized by augmenting the input with a text string that may include candidate examples from the dataset, and cues for the model to complete the sequence.
% such that filling the \mask token in this text outputs the true class. 
% This appended text string is commonly called a \emph{prompt template} and the projection from the infilled token to class label is done via a list of \emph{candidate answers}. For instance, in the task of movie review sentiment classification, a viable \emph{template} would be \emph{"Overall, this movie is \emph{\mask}"}. The  \emph{candidate answers} would be used to map positive words such as \{\emph{great, good}\} to class 1 and negative words such as \{\emph{bad, terrible}\} to class 0. The final prediction would be made based on which of these words the language model finds more probable, given the input.
% \dd{The example is helpful but is too verbose, I'd say remove it, and instead include a high-level introductory figure.}\textcolor{blue}{do we want a second figure to explain this?}
However, the advantage of \emph{prompting} has only been investigated in the context of zero-shot and few-shot learning, or when the parameters of the underlying language model are either kept frozen or allow modifying a few layers. 
Further, prompting has generally been seen as an effective strategy with large-scale models~\cite{lester-etal-2021-power} which are inaccessible to most users because of their high compute and memory requirements. We evaluate models trained via \ourPrompt in the context of full data fine-tuning (and has not been considered in prior work to the best of our knowledge).

Despite pre-training their representations on large amounts of text data, the models fine-tuned on downstream tasks using \linearFT break under adversarial input perturbations~\citep{Jin_Jin_Zhou_Szolovits_2020,li-etal-2020-bert-attack,morris-etal-2020-textattack}. It has been found that small changes in the input text, such as replacement with synonyms~\citep{ebrahimi-etal-2018-hotflip}, and adversarial misspellings~\citep{ebrahimi-etal-2018-adversarial,pruthi-etal-2019-combating}
 drastically reduce the robustness of text classification models. 
% \dd{A different way to tell our story is to start from here. Say that prompting has solely been investigated in zero-shot context, but there's no reason to not finetune through prompts, and we tried it and it not just performs well, but is more robust because ...} 
% \zk{I agree with Danish.  I think the intro here is too verbose and takes too long to get the “main” point that you’re considering robustness of prompts.}

In this work, 
we demonstrate that model-tuning via prompting (\ourPromptns) remarkably improves the adversarial robustness of models  as compared to fine-tuning with an MLP head (\linearFTns).
% we demonstrate that classification in the traditional supervised learning paradigm of fine-tuning  can gain significantly in terms of adversarial robustness when performed via prompting, and we will denote this by \ourPrompt to disambiguate with other forms of prompting. 
% \dd{We can simplify the punchline here by saying that ``We demonstrate that finetuning via prompting improves the adversarial robustness of models remarkably as compared to finetuning a linear head".}
% \todomr{Please correct the numbers here.}
Surprisingly, ~\ourPromptns, which does not utilize any sort of (i) adversarial training, and (ii) prompt engineering  already yields higher adversarial robustness compared to the state-of-the-art methods utilizing adversarial training by an average of $3.5\%$ across three tasks, two models and two attacks (Section ~\ref{subsec:results}). This is especially of interest because these models achieve similar clean accuracy, suggesting that these models have significantly higher effective robustness.
Moreover, we find that combining \ourPrompt with single-step adversarial training (in the model's embedding space) can further boost adversarial robustness, resulting in combined robustness gains of over $10\%$ from the current state-of-art baselines. This happens without any loss in clean accuracy, indicating how the objective of adversarial training aligns well with \ourPromptns. 
% \dd{Somewhere here or above, we should also talk about clean accuracies.}
% dd{Before getting to implications}

In addition to adversarial robustness, we show that \ourPrompt as a method for classification is more (i) sample efficient, and (ii) has higher effective robustness than \linearFT (Section ~\ref{subsec:additional-advantages}). That is,  \ourPrompt requires much fewer training samples to achieve the same clean accuracy; and for any given clean accuracy, 
the robust accuracy of \ourPrompt is higher than when predicting via \linearFTns.
Through ablation studies (Section \ref{subsec:ablation}), we find that (i) unlike the few-shot learning paradigm, having multiple candidate answers has a negligible impact on the robustness of \ourPromptns; and 
adding multiple templates makes it harder for the adversary to fool multiple inputs simultaneously.

% Particularly, we find that:
To explain our observations, we test a set of hypotheses (Section \ref{sec:hypothesis}), 
including 
(i) \emph{pretraining task alignment}---can the gains in robustness be attributed to the alignment between the fine-tuning and pertaining tasks?;
(ii) \emph{extra parameter vulnerability}---is adding a randomly initialized linear head the source of adversarial vulnerability?; and
(iii) \emph{label semanticity alignment}---are predictions by \ourPrompt more robust because the candidate answer is semantically connected to the class label? 
Through experiments designed to test each of these hypotheses, we find that (i) absent-pretraining, \ourPrompt and \linearFT have similar robustness performance, supporting the hypothesis of pretraining task alignment; (ii) adding extra uninitialized parameters to \ourPrompt leads to a sharp drop in robustness, whereas removing the dense $(768, 768)$ randomly initialized weight matrix from \linearFT helps increase the robustness of the model significantly; (iii) even random candidate answers such as `jack', and `jill' result in similar robustness gains, suggesting that in the fine-tuning domain, contrary to zero-shot and few-shot setting, the candidate answers do not matter.




We also perform a user study (Section \ref{sec:discussion}) to assess the quality of adversarial examples on which \ourPrompt + Adv fails to correctly classify adversarial examples. We find that in 57\% cases, users were able to identify that the input had been perturbed, and in 85\% cases, the adversarially perturbed sentence had ambiguous or incorrect label post-modification.
\dd{Does this mean that for 85\% of the examples, the new label (assigned after manipulation) and the original label (in the original dataset) was different. If yes, is it fair to even treat the original ground truth as true anymore?} \zk{What is baseline performance on the cases where MVP + Adv does correctly classify?}
This suggests that \ourPrompt is significantly robust, and future work will benefit from developing better evaluation strategies for the robustness of NLP models.
Note that all our observations are in the full data fine-tuning regime and offer a new outlook as opposed to past work which has focused on few-shot or zero-shot prompting. 
% \ddc{In summary, our contributions are:}{}
% \begin{enumerate}
% % \item We provide a benchmark evaluation for prior defenses, finding that many of the claims made for robustness are inflated, and those for standard models are more than stated.
% \item \ddc{We demonstrate the robustness of model-tuning via prompts (\ourPromptns) in the conventional supervised training paradigm.}{}

% \item \ddc{We find that \ourPrompt is significantly more sample efficient and effectively robust as opposed to \linearFT.}{}

% \item \ddc{Through a series of ablations, we find that the big gains of adversarial robustness due to \ourPrompt are attributable to the pre-training task alignment, and the absence of any new random parameters in the model.}{}

% \item 
% \ddc{We perform a user study highlighting the need for better evaluation metrics to reliably evaluate the robustness of NLP models.}{}

% \end{enumerate}


==> sections/abstract-sub.tex <==
In recent years,
NLP practitioners have converged
on the following practice:
(i) import an off-the-shelf pretrained (masked) language model;
(ii) append a multilayer perceptron atop the CLS token's hidden representation
(with randomly initialized weights);
and (iii) fine-tune the entire model on a downstream task (MLP-FT).
This 
procedure 
has 
produced massive gains 
on standard NLP benchmarks,
but these models remain brittle, even to 
mild adversarial perturbations.
In this work, we demonstrate surprising gains 
in adversarial robustness enjoyed by 
Model-tuning Via Prompts (MVP),
an alternative method of adapting to downstream tasks.
Rather than appending an MLP head to make output prediction, MVP appends a prompt template to the input, and makes prediction via text infilling/completion.
Across three classification datasets,
MVP improves performance against adversarial 
substitutions  by an average of 8% 
over standard methods and even outperforms 
adversarial training-based state-of-art defenses by 3.5%.
By combining MVP with adversarial training, 
we achieve further improvements in adversarial robustness
while maintaining performance on unperturbed examples. We further demonstrate the efficacy of MVP on a paraphrase detection task and a 14-class classification task. 
Finally, we conduct ablations to investigate 
the mechanism underlying these gains.
Notably, we find that the main causes of vulnerability of MLP-FT 
can be attributed to the misalignment between pre-training and fine-tuning tasks, 
and the randomly initialized MLP parameters.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}



==> sections/reviews.tex <==
\section{ICML 2023 Reviews}

We had submitted our work to ICML, and received scores of 6,6,4 (Weak Accept, Weak Accept, Borderline Reject). The paper did not go through at the conference. The reviews for the same are presented in the screenshots below. 

\subsection{Revisions Made}
The main concerns among reviewers were about (i) the limited scope of our experiments (R1, R2), and (ii) how our work differentiates from the prior literature (R2, R3).

\begin{enumerate}
    \item To address the first concern, we have extended the scope of our analysis to include \textbf{two new attack strategies} and\textbf{ two additional tasks}. These new experiments provide additional evidence to support our original findings about the adversarial robustness conferred by model-tuning via prompts (MVP) as opposed to the conventional approach of MLP-FT. We would like to highlight that our benchmarking effort, comparatively, is more extensive than many past published analyses (for example \cite{li-etal-2021-searching}).


    \item For the second concern, we have updated our draft to clarify how our work relates to past work. Briefly, most prior work that studies the advantages of prompting on robustness is either focused on out-of-domain generalization, or is limited to few- or zero-shot setups. We are the first to study the adversarial robustness of models that are fine-tuned via prompts. Using model tuning via prompts, we obtain large and noteworthy gains. Coupled with adversarial training, the resulting models achieve a new state-of-the-art performance, outperforming existing defenses by 7\% percent on average. We are also the first to consider an extensive set of hypotheses to explain such a phenomenon.
\end{enumerate}


\begin{figure*}[b]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/r1.png}
\end{figure*}
\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figures/r2.png}
\end{figure*}
\begin{figure*}[t]
    \includegraphics[width=\textwidth]{figures/r3.png}
\end{figure*}

\clearpage

==> tables/main_table.tex <==
\begin{table*}[t]
% \footnotesize
\centering
\scalebox{\tablescale}{

\begin{tabular}{@{}lclccrcc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{AG News}} &\\
\toprule
 & \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
 & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
 \midrule
\linearFT  & 93.76 \footnotesize $\pm$ 0.46 & 37.53 \footnotesize $\pm$ 0.67 & 58.97 \footnotesize $\pm$ 0.67 & 94.50 \footnotesize $\pm$ 0.40 & 42.86 \footnotesize $\pm$ 0.74 & 61.80 \footnotesize $\pm$ 0.30 \\
\linearFT + Adv & 93.23 \footnotesize $\pm$ 0.23 & 44.34 \footnotesize $\pm$ 0.98 & 64.12 \footnotesize $\pm$ 0.23 & 94.40 \footnotesize $\pm$ 0.61 & 47.67 \footnotesize $\pm$ 0.51 & 65.60 \footnotesize $\pm$ 0.78 \\
Free LB++ & 93.40 \footnotesize $\pm$ 0.20 & 43.53 \footnotesize $\pm$ 0.21 & 63.43 \footnotesize $\pm$ 0.78 & 94.37 \footnotesize $\pm$ 0.68 & 46.93 \footnotesize $\pm$ 1.60 & 65.56 \footnotesize $\pm$ 1.00 \\
AMDA & 92.83 \footnotesize $\pm$ 0.55 & 41.80 \footnotesize $\pm$ 0.87 & 62.63 \footnotesize $\pm$ 1.04 & 94.10 \footnotesize $\pm$ 0.62 & 44.30 \footnotesize $\pm$ 1.41 & 62.90 \footnotesize $\pm$ 0.51 \\
InfoBERT & 93.83 \footnotesize $\pm$ 0.30 & 43.97 \footnotesize $\pm$ 1.60 & 64.08 \footnotesize $\pm$ 0.78 & 94.50 \footnotesize $\pm$ 0.89 & 48.00 \footnotesize $\pm$ 2.25 & 65.63 \footnotesize $\pm$ 1.20 \\
 \ourPrompt & 93.70 \footnotesize $\pm$ 0.46 & \uline{46.27 \footnotesize {$\pm$ 1.15}} & \uline{65.97 \footnotesize {$\pm$ 0.35}} & 94.33 \footnotesize $\pm$ 0.21 & \uline{51.46 \footnotesize {$\pm$ 2.06}} & \uline{68.73 \footnotesize {$\pm$ 0.70}} \\
\ourPrompt + Adv  & 93.97 \footnotesize $\pm$ 0.59 & \textbf{53.73 \footnotesize $\pm$ 0.06} & \textbf{69.17 \footnotesize $\pm$ 1.27} & 94.43 \footnotesize $\pm$ 0.81 & \textbf{62.73 \footnotesize $\pm$ 2.35} & \textbf{75.33 \footnotesize $\pm$ 1.60}  \\
\toprule
& \multicolumn{6}{c}{\textbf{BoolQ}} &\\ 
\toprule
& \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
 & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
 \midrule
 \linearFT  & 71.13 \footnotesize $\pm$ 1.34 & 21.77 \footnotesize $\pm$ 4.38 & 36.80 \footnotesize $\pm$ 3.00 & 80.60 \footnotesize $\pm$ 1.56 & 28.23 \footnotesize $\pm$ 1.68 & 38.36 \footnotesize $\pm$ 1.09 \\
\linearFT + Adv & 70.98 \footnotesize $\pm$ 0.91 & 29.78 \footnotesize $\pm$ 0.78 & 42.78 \footnotesize $\pm$ 1.34 & 78.86 \footnotesize $\pm$ 1.26 & 39.00 \footnotesize $\pm$ 0.72 & 44.40 \footnotesize $\pm$ 1.25 \\
Free LB++ & 70.73 \footnotesize $\pm$ 0.15 & 29.50 \footnotesize $\pm$ 0.61 & 42.83 \footnotesize $\pm$ 0.63 & 80.63 \footnotesize $\pm$ 0.49 & 37.27 \footnotesize $\pm$ 1.47 & 43.23 \footnotesize $\pm$ 1.05\\
AMDA & 71.06 \footnotesize $\pm$ 0.91 & 25.37 \footnotesize $\pm$ 0.76 & 41.60 \footnotesize $\pm$ 0.61 & 79.20 \footnotesize $\pm$ 0.95 & 32.03 \footnotesize $\pm$ 0.32 & 41.10 \footnotesize $\pm$ 0.20 \\
InfoBERT & 71.77 \footnotesize $\pm$ 0.55 & 29.86 \footnotesize $\pm$ 0.25 & 42.60 \footnotesize $\pm$ 0.56 & 81.50 \footnotesize $\pm$ 0.70 & 38.07 \footnotesize $\pm$ 1.37 & 42.47 \footnotesize $\pm$ 0.96 \\
\ourPrompt  & 71.43 \footnotesize $\pm$ 1.00& \uline{31.13 \footnotesize {$\pm$ 1.27}} & \uline{44.40 \footnotesize {$\pm$ 2.78}} & 82.00 \footnotesize $\pm$ 0.60 & \uline{42.93 \footnotesize {$\pm$ 0.57}} & \uline{49.86 \footnotesize {$\pm$ 1.67}} \\
\ourPrompt + Adv & 71.27 \footnotesize $\pm$ 0.72 & \textbf{43.10 \footnotesize $\pm$ 0.70} & \textbf{49.93 \footnotesize $\pm$ 0.90} & 81.07 \footnotesize $\pm$ 0.60 & \textbf{52.23 \footnotesize $\pm$ 1.62} & \textbf{56.46 \footnotesize $\pm$ 1.60} \\ \toprule
& \multicolumn{6}{c}{\textbf{SST2}} &\\
\toprule
& \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
 & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
 \midrule
\linearFT  & 91.97 \footnotesize $\pm$ 0.20 & 38.32 \footnotesize $\pm$ 1.01 & 60.41 \footnotesize $\pm$ 0.48 & 93.58 \footnotesize $\pm$ 0.40 & 40.25 \footnotesize $\pm$ 0.94 & 65.37 \footnotesize $\pm$ 0.28 \\
\linearFT + Adv & 90.98 \footnotesize $\pm$ 0.34 & 42.89 \footnotesize $\pm$ 1.23 & 62.34 \footnotesize $\pm$ 0.52 & 93.63 \footnotesize $\pm$ 0.63 & 44.04 \footnotesize $\pm$ 1.24 & 68.47 \footnotesize $\pm$ 1.47 \\
Free LB++ & 92.16 \footnotesize $\pm$ 0.84 & 42.25 \footnotesize $\pm$ 1.01 & 63.05 \footnotesize $\pm$ 0.71 & 94.05 \footnotesize $\pm$ 0.09 & 43.37 \footnotesize $\pm$ 1.00 & 67.15 \footnotesize $\pm$ 0.64 \\
AMDA & 92.18 \footnotesize $\pm$ 0.89 & 41.72 \footnotesize $\pm$ 0.57 & 60.96 \footnotesize $\pm$ 0.44 & 93.84 \footnotesize $\pm$ 0.42 & 41.85 \footnotesize $\pm$ 0.46 & 66.06 \footnotesize $\pm$ 0.17 \\
InfoBERT & 91.79 \footnotesize $\pm$ 0.67 & 43.15 \footnotesize $\pm$ 0.81 & 64.69 \footnotesize $\pm$ 0.66 & 94.00 \footnotesize $\pm$ 0.40 & 43.63 \footnotesize $\pm$ 0.52 & 66.58 \footnotesize $\pm$ 1.77 \\
\ourPrompt & 91.78 \footnotesize $\pm$ 0.46 & \uline{44.67 \footnotesize {$\pm$ 0.76}} & \uline{65.16 \footnotesize {$\pm$ 0.05}} & 93.92 \footnotesize $\pm$ 0.70 & \uline{46.88 \footnotesize {$\pm$ 0.50}} & \uline{69.80 \footnotesize {$\pm$ 0.51}}\\
\ourPrompt+ Adv & 91.80 \footnotesize $\pm$ 0.74 & \textbf{47.67 \footnotesize $\pm$ 0.58} & \textbf{67.77 \footnotesize $\pm$ 0.39} & 93.82 \footnotesize $\pm$ 0.12 & \textbf{53.78 \footnotesize $\pm$ 0.72}& \textbf{71.73 \footnotesize $\pm$ 0.85} \\ \bottomrule
\end{tabular}
}
\caption{
Adversarial performance of BERT-base and RoBERTa-base models on $3$ datasets averaged over $3$ seeds.
% Adversarial performance of BERT-base and RoBERTa-base models on $3$ different datasets. All accuracy values are reported for a fixed test set of size 1000 and are averaged over $3$ different seeds. The highest accuracies are bolded, and the second-best are  underlined. 
% % We observe that models tuned via prompts 
% \ourPrompt is the most robust, and preserves (or improves) the clean accuracy.
}
\label{tab:acc-main}
\end{table*}

% \begin{tabular}{@{}lclccrcc@{}}
% \toprule
% & \multicolumn{6}{c}{\textbf{AG News}} &\\
% \toprule
%  & \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
%  & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
%  \midrule
% \linearFT  & 93.7 \footnotesize $\pm$ 0.4 & 37.5 \footnotesize $\pm$ 0.6 & 58.9 \footnotesize $\pm$ 0.6 & 94.5 \footnotesize $\pm$ 0.4 & 42.8 \footnotesize $\pm$ 0.7 & 61.8 \footnotesize $\pm$ 0.3 \\
% \linearFT + Adv & 93.2 \footnotesize $\pm$ 0.2 & 44.3 \footnotesize $\pm$ 0.9 & 64.1 \footnotesize $\pm$ 0.2 & 94.4 \footnotesize $\pm$ 0.6 & 47.6 \footnotesize $\pm$ 0.5 & 65.6 \footnotesize $\pm$ 0.7 \\
% Free LB++ & 93.4 \footnotesize $\pm$ 0.2 & 43.5 \footnotesize $\pm$ 0.2 & 63.4 \footnotesize $\pm$ 0.7 & 94.3 \footnotesize $\pm$ 0.6 & 46.9 \footnotesize $\pm$ 1.6 & 65.5 \footnotesize $\pm$ 1.0 \\
% AMDA & 92.8 \footnotesize $\pm$ 0.5 & 41.8 \footnotesize $\pm$ 0.8 & 62.6 \footnotesize $\pm$ 1.0 & 94.1 \footnotesize $\pm$ 0.6 & 44.3 \footnotesize $\pm$ 1.4 & 62.9 \footnotesize $\pm$ 0.5 \\
% InfoBERT & 93.8 \footnotesize $\pm$ 0.3 & 43.9 \footnotesize $\pm$ 1.6 & 64.0 \footnotesize $\pm$ 0.7 & 94.5 \footnotesize $\pm$ 0.8 & 48.0 \footnotesize $\pm$ 2.2 & 65.6 \footnotesize $\pm$ 1.2 \\
%  \ourPrompt & 93.7 \footnotesize $\pm$ 0.4 & \uline{46.2 \footnotesize {$\pm$ 1.1}} & \uline{65.9 \footnotesize {$\pm$ 0.3}} & 94.3 \footnotesize $\pm$ 0.2 & \uline{51.4 \footnotesize {$\pm$ 2.0}} & \uline{68.7 \footnotesize {$\pm$ 0.7}} \\
% \ourPrompt + Adv  & 93.9 \footnotesize $\pm$ 0.5 & \textbf{53.7 \footnotesize $\pm$ 0.1} & \textbf{69.1 \footnotesize $\pm$ 1.2} & 94.4 \footnotesize $\pm$ 0.8 & \textbf{62.7 \footnotesize $\pm$ 2.3} & \textbf{75.3 \footnotesize $\pm$ 1.6}  \\
% \toprule
% & \multicolumn{6}{c}{\textbf{BoolQ}} &\\ 
% \toprule
% & \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
%  & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
%  \midrule
%  \linearFT  & 71.1 \footnotesize $\pm$ 1.3 & 21.7 \footnotesize $\pm$ 4.3 & 36.8 \footnotesize $\pm$ 3.0 & 80.6 \footnotesize $\pm$ 1.5 & 28.2 \footnotesize $\pm$ 1.6 & 38.3 \footnotesize $\pm$ 1.0 \\
% \linearFT + Adv & 70.9 \footnotesize $\pm$ 0.9 & 29.7 \footnotesize $\pm$ 0.7 & 42.7 \footnotesize $\pm$ 1.3 & 78.8 \footnotesize $\pm$ 1.2 & 39.0 \footnotesize $\pm$ 0.7 & 44.4 \footnotesize $\pm$ 1.2 \\
% Free LB++ & 70.7 \footnotesize $\pm$ 0.1 & 29.5 \footnotesize $\pm$ 0.6 & 42.8 \footnotesize $\pm$ 0.6 & 80.6 \footnotesize $\pm$ 0.5 & 37.2 \footnotesize $\pm$ 1.4 & 43.2 \footnotesize $\pm$ 1.0\\
% AMDA & 71.0 \footnotesize $\pm$ 0.9 & 25.3 \footnotesize $\pm$ 0.7 & 41.6 \footnotesize $\pm$ 0.6 & 79.2 \footnotesize $\pm$ 0.9 & 32.0 \footnotesize $\pm$ 0.3 & 41.1 \footnotesize $\pm$ 0.2 \\
% InfoBERT & 71.7 \footnotesize $\pm$ 0.5 & 29.8 \footnotesize $\pm$ 0.2 & 42.6 \footnotesize $\pm$ 0.5 & 81.5 \footnotesize $\pm$ 0.7 & 38.0 \footnotesize $\pm$ 1.3 & 42.4 \footnotesize $\pm$ 0.9 \\
% \ourPrompt  & 71.4 \footnotesize $\pm$ 1.0 & \uline{31.1 \footnotesize {$\pm$ 1.2}} & \uline{44.4 \footnotesize {$\pm$ 2.7}} & 82.0 \footnotesize $\pm$ 0.6 & \uline{42.9 \footnotesize {$\pm$ 0.5}} & \uline{49.8 \footnotesize {$\pm$ 1.6}} \\
% \ourPrompt + Adv & 71.2 \footnotesize $\pm$ 0.7 & \textbf{43.1 \footnotesize $\pm$ 0.7} & \textbf{49.9 \footnotesize $\pm$ 0.9} & 81.0 \footnotesize $\pm$ 0.6 & \textbf{52.2 \footnotesize $\pm$ 1.6} & \textbf{56.4 \footnotesize $\pm$ 1.6} \\ \toprule
% & \multicolumn{6}{c}{\textbf{SST-2}} &\\
% \toprule
% & \multicolumn{3}{c}{BERT-Base} & \multicolumn{3}{c}{RoBERTa-Base} &   \\ \midrule
%  & \multicolumn{1}{l}{Clean Acc} & \multicolumn{1}{l}{TextFooler} & \multicolumn{1}{l}{TextBugger} & Clean Acc & TextFooler & TextBugger & \\
%  \midrule
% \linearFT  & 91.9 \footnotesize $\pm$ 0.2 & 38.3 \footnotesize $\pm$ 1.0 & 60.4 \footnotesize $\pm$ 0.4 & 93.5 \footnotesize $\pm$ 0.4 & 40.2 \footnotesize $\pm$ 0.9 & 65.3 \footnotesize $\pm$ 0.2 \\
% \linearFT + Adv & 90.9 \footnotesize $\pm$ 0.3 & 42.9 \footnotesize $\pm$ 1.2 & 62.3 \footnotesize $\pm$ 0.5 & 93.6 \footnotesize $\pm$ 0.6 & 44.0 \footnotesize $\pm$ 1.2 & 68.4 \footnotesize $\pm$ 1.4 \\
% Free LB++ & 92.1 \footnotesize $\pm$ 0.8 & 42.2 \footnotesize $\pm$ 1.0 & 63.0 \footnotesize $\pm$ 0.7 & 94.0 \footnotesize $\pm$ 0.1 & 43.3 \footnotesize $\pm$ 1.0 & 67.1 \footnotesize $\pm$ 0.6 \\
% AMDA & 92.1 \footnotesize $\pm$ 0.8 & 41.7 \footnotesize $\pm$ 0.5 & 60.9 \footnotesize $\pm$ 0.4 & 93.8 \footnotesize $\pm$ 0.4 & 41.8 \footnotesize $\pm$ 0.4 & 66.0 \footnotesize $\pm$ 0.1 \\
% InfoBERT & 91.8 \footnotesize $\pm$ 0.6 & 43.1 \footnotesize $\pm$ 0.8 & 64.7 \footnotesize $\pm$ 0.6 & 94.0 \footnotesize $\pm$ 0.4 & 43.6 \footnotesize $\pm$ 0.5 & 66.5 \footnotesize $\pm$ 1.7 \\
% \ourPrompt & 91.7 \footnotesize $\pm$ 0.4 & \uline{44.6 \footnotesize {$\pm$ 0.7}} & \uline{65.1 \footnotesize {$\pm$ 0.1}} & 93.9 \footnotesize $\pm$ 0.7 & \uline{46.8 \footnotesize {$\pm$ 0.5}} & \uline{69.8 \footnotesize {$\pm$ 0.5}}\\
% \ourPrompt+ Adv & 91.8 \footnotesize $\pm$ 0.7 & \textbf{47.6 \footnotesize $\pm$ 0.5} & \textbf{67.7 \footnotesize $\pm$ 0.3} & 93.8 \footnotesize $\pm$ 0.1 & \textbf{53.7 \footnotesize $\pm$ 0.7}& \textbf{71.7 \footnotesize $\pm$ 0.8} \\ \bottomrule
% \end{tabular}
% }
% \caption{Adversarial robustness results on AG News, SST-2 and BoolQ Dataset for BERT-Base and RoBERTa-Base Models. \zk{I feel like a bar chart is quite a bit better for presenting these results; You can include the full tables in the appendix?} All experiments are run on 3 different seeds and the performance is reported over a fixed test set of size 1000. The best-performing robust accuracies are bolded and the second best robust accuracies are underlined.}
% \label{tab:acc-main}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table*}[]
% \centering
% \begin{tabular}{@{}lllllll@{}}
% \toprule
%  & \multicolumn{3}{c}{TextFooler} & \multicolumn{3}{c}{TextBugger} \\ \midrule
%  & Clean Acc & \# queries & Robust Acc & Clean Acc & \# queries & Robust Acc \\
% \linearFT  & 94.50 \footnotesize $\pm$ 0.40 & 266.90 \footnotesize $\pm$ 5.01 & 42.86 \footnotesize $\pm$ 0.74 & 94.50 \footnotesize $\pm$ 0.40 & 89.98 \footnotesize $\pm$ 1.72 & 61.80 \footnotesize $\pm$ 0.30 \\
% Free LB++ & 94.37 \footnotesize $\pm$ 0.68 & 245.55 \footnotesize $\pm$ 11.16 & 46.93 \footnotesize $\pm$ 1.60 & 94.37 \footnotesize $\pm$ 0.68 & 101.17 \footnotesize $\pm$ 3.39 & 65.56 \footnotesize $\pm$ 1.00 \\
% Mixtext & 94.10 \footnotesize $\pm$ 0.62 & 216.42 \footnotesize $\pm$ 6.20 & 44.30 \footnotesize $\pm$ 1.41 & 94.10 \footnotesize $\pm$ 0.62 & 93.73 \footnotesize $\pm$ 2.76 & 62.90 \footnotesize $\pm$ 0.51 \\
% InfoBert & 94.50 \footnotesize $\pm$ 0.89 & 227.97 \footnotesize $\pm$ 17.92 & 48.00 \footnotesize $\pm$ 2.25 & 94.50 \footnotesize $\pm$ 0.89 & 100.69 \footnotesize $\pm$ 3.90 & 65.63 \footnotesize $\pm$ 1.20 \\
% \ourPrompt & 94.33 \footnotesize $\pm$ 0.21 & 301.75 \footnotesize $\pm$ 16.84 & {\ul 51.46 \footnotesize $\pm$ 2.06} & 94.33 \footnotesize $\pm$ 0.21 & 97.19 \footnotesize $\pm$ 5.05 & {\ul 68.73 \footnotesize $\pm$ 0.70} \\
% \ourPrompt + Adv & 94.43 \footnotesize $\pm$ 0.81 & 302.49 \footnotesize $\pm$ 7.41 & \textbf{62.73 \footnotesize $\pm$ 2.35} & 94.43 \footnotesize $\pm$ 0.81 & 92.17 \footnotesize $\pm$ 1.91 & \textbf{75.33 \footnotesize $\pm$ 1.60} \\ \bottomrule
% \end{tabular}
% \caption{Robust accuracy of various Defenders on the AGNews dataset}
% \label{tab:ag_news}
% \end{table*}

==> tables/main_table_fig.tex <==
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
% \\
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
% \includegraphics[width=0.33\linewidth]{figures/figure.pdf}
%   \caption{Variation of clean and robust accuracies on the AG News dataset with change in amount of training data available. The train set size (x-axis) uses a log scale.  All the models are trained on the RoBERTa-Base backbone. The size of the complete AG News training set is 120k }
%   \label{fig:main-table-fig}
% \end{figure*}

==> tables/main_table_option_2.tex <==
\begin{table*}[t]
\centering
\scalebox{\tablescale}{
\begin{tabular}{@{}lccccc@{}}
\toprule
             & \multicolumn{5}{c}{SST2}                                                  \\\toprule
             & Clean Acc      & TextFooler   & TextBugger   & BertAttack  & Misspellings       \\\midrule
\linearFT       & 93.6 \footnotesize $\pm$0.4    & 40.2 \footnotesize $\pm$0.9 & 65.4 \footnotesize $\pm$0.3 & 70.3 \footnotesize $\pm$0.9 & 45.2\footnotesize $\pm$1.1   \\
\linearFT + Adv & 93.6 \footnotesize $\pm$0.6    & 44.0 \footnotesize $\pm$1.2 & 68.5 \footnotesize $\pm$1.5 & 74.3\footnotesize $\pm$0.8  & 49.3 \footnotesize $\pm$0.3  \\
Free LB++    & 94.0 \footnotesize $\pm$0.1    & 43.4 \footnotesize $\pm$1.0 & 67.2 \footnotesize $\pm$0.6 & 76.2 \footnotesize $\pm$0.6 & 50.4\footnotesize $\pm$1.1   \\
MADA         & 93.8 \footnotesize $\pm$0.4    & 41.8 \footnotesize $\pm$0.5 & 66.1 \footnotesize $\pm$0.2 & 74.2 \footnotesize $\pm$0.2 & 45.4 \footnotesize $\pm$0.4  \\
InfoBert     & 94.0 \footnotesize $\pm$0.4    & 43.6 \footnotesize $\pm$0.5 & 66.6 \footnotesize $\pm$1.8 & 76.1 \footnotesize $\pm$0.6 & 47.1 \footnotesize $\pm$0.4  \\
\ourPrompt       & 93.9 \footnotesize $\pm$0.7    & \uline{46.9 \footnotesize {$\pm$0.5}} & 69.8 \footnotesize $\pm$0.5 & 78.1 \footnotesize $\pm$0.9 & 50.5 \footnotesize $\pm$0.7  \\
\ourPrompt + Adv & 93.8 \footnotesize $\pm$0.1    & 53.8 \footnotesize $\pm$0.7 & 71.7 \footnotesize $\pm$0.8 & 81.7 \footnotesize $\pm$0.7 & 54.9 \footnotesize $\pm$1.3  \\
\toprule
             & \multicolumn{5}{c}{AG News}                                               \\\toprule
             & Clean Acc      & TextFooler   & TextBugger   & BertAttack  & Misspellings       \\\midrule
\linearFT       & 94.5 \footnotesize $\pm$0.4   & 42.9 \footnotesize $\pm$0.7 & 61.8 \footnotesize $\pm$0.3 & 79.1 \footnotesize $\pm$1.3 & 76.8 \footnotesize $\pm$1.3  \\
\linearFT + Adv & 94.4 \footnotesize $\pm$0.6    & 47.7 \footnotesize $\pm$0.5 & 65.6 \footnotesize $\pm$0.8 & 81.1\footnotesize $\pm$1.0  & 78.6 \footnotesize $\pm$0.8 \\
Free LB++    & 94.4 \footnotesize $\pm$0.7   & 46.9 \footnotesize $\pm$1.6 & 65.5 \footnotesize $\pm$1.0 & 81.4 \footnotesize $\pm$0.9 & 80.1 \footnotesize $\pm$1.3  \\
MADA         & 94.1 \footnotesize $\pm$0.6   & 44.3 \footnotesize $\pm$1.4 & 62.9 \footnotesize $\pm$0.5 & 80.4 \footnotesize $\pm$0.2 & 77.1 \footnotesize $\pm$0.4  \\
InfoBert     & 94.5 \footnotesize $\pm$0.9   & 48.0 \footnotesize $\pm$2.2 & 65.6 \footnotesize $\pm$1.2 & 82.4\footnotesize $\pm$1.2  & 80.4\footnotesize $\pm$1.4   \\
\ourPrompt       & 94.3 \footnotesize $\pm$0.2   & 51.5 \footnotesize $\pm$2.1 & 68.7 \footnotesize $\pm$0.7 & 85.3 \footnotesize $\pm$1.3 & 82.7 \footnotesize $\pm$0.7  \\
\ourPrompt + Adv & 94.4 \footnotesize $\pm$0.8   & 62.7 \footnotesize $\pm$2.4 & 75.3 \footnotesize $\pm$1.6 & 88.2 \footnotesize $\pm$0.9 & 86.6 \footnotesize $\pm$0.6  \\
\toprule
             & \multicolumn{5}{c}{BoolQ}                                                 \\\toprule
             & Clean Acc      & TextFooler   & TextBugger   & BertAttack  & Misspellings       \\\midrule
\linearFT       & 80.6 \footnotesize $\pm$1.5   & 28.2 \footnotesize $\pm$1.7 & 38.3 \footnotesize $\pm$1.0 & 54.3 \footnotesize $\pm$1.8 & 55.2\footnotesize $\pm$1.2   \\
\linearFT + Adv & 78.9 \footnotesize $\pm$1.2   & 39.0 \footnotesize $\pm$0.7 & 44.4 \footnotesize $\pm$1.2 & 57.4 \footnotesize $\pm$0.9 & 57.3 \footnotesize $\pm$1.3  \\
Free LB++    & 80.6 \footnotesize $\pm$0.4   & 37.2 \footnotesize $\pm$1.4 & 43.2 \footnotesize $\pm$1.0 & 58.3 \footnotesize $\pm$0.5 & 58.0\footnotesize $\pm$1.1   \\
MADA         & 79.2 \footnotesize $\pm$0.9   & 32.0 \footnotesize $\pm$0.3 & 41.1 \footnotesize $\pm$0.2 & 57.9 \footnotesize $\pm$0.2 & 56.4 \footnotesize $\pm$0.2  \\
InfoBert     & 81.5 \footnotesize $\pm$0.7   & 38.0 \footnotesize $\pm$1.3 & 42.4 \footnotesize $\pm$0.9 & 59.1 \footnotesize $\pm$0.5 & 59.1 \footnotesize $\pm$1.4   \\
\ourPrompt       & 82.0 \footnotesize $\pm$0.6   & 42.9 \footnotesize $\pm$0.5 & 49.8 \footnotesize $\pm$1.6 & 64.1 \footnotesize $\pm$0.7 & 60.1 \footnotesize $\pm$1.6  \\
\ourPrompt + Adv & 81.1 \footnotesize $\pm$0.6   & 52.2 \footnotesize $\pm$1.6 & 56.4 \footnotesize $\pm$1.6 & 68.2 \footnotesize $\pm$0.6 & 64.3 \footnotesize $\pm$0.3  \\
\bottomrule
\end{tabular}
}
\caption{Adversarial performance of RoBERTa-base model on $3$ different datasets. All accuracy values are reported for a fixed test set of size 1000 and are averaged over $3$ different seeds. The highest accuracies are bolded, and the second-best is  underlined. 
% We observe that models tuned via prompts 
}
\label{tab:acc-main}
\end{table*}
